DP-Dueling: Learning from Preference Feedback without Compromising User Privacy

We consider the well-studied dueling bandit problem, where a learner aims to identify near-optimal actions using pairwise comparisons, under the constraint of differential privacy. We consider a general class of utility-based preference matrices for large (potentially unbounded) decision spaces and give the first differentially private dueling bandit algorithm for active learning with user preferences. Our proposed algorithms are computationally efficient with near-optimal performance, both in terms of the private and non-private regret bound. More precisely, we show that when the decision space is of finite size $K$, our proposed algorithm yields order optimal $O\Big(\sum_{i = 2}^K\log\frac{KT}{\Delta_i} + \frac{K}{\epsilon}\Big)$ regret bound for pure $\epsilon$-DP, where $\Delta_i$ denotes the suboptimality gap of the $i$-th arm. We also present a matching lower bound analysis which proves the optimality of our algorithms. Finally, we extend our results to any general decision space in $d$-dimensions with potentially infinite arms and design an $\epsilon$-DP algorithm with regret $\tilde{O} \left( \frac{d^6}{\kappa \epsilon } + \frac{ d\sqrt{T }}{\kappa} \right)$, providing privacy for free when $T \gg d$.

==> algorithm.tex <==
\section{Adaptive Algorithm Stochastic Case (Fixed $\P$)}
\label{sec:alg_stoc}

In this section we first propose an algorithm that is adaptive to the underlying preference structure $\P$. More precisely, the algorithm can adapt itself to the \tot \, structure if $\P$ respects total ordering, yielding an optimal regret bound of $\tO\big( \sum_{k = 1}^{K} \frac{\log T}{\Delta_i} \big)$. On the other hand, under only \cw \, structure it yields a regret guarantee of $\tO\big( \sum_{k = 1}^{K} K\frac{\log T}{\Delta_i} \big)$, which is tight up to a constant factor of $K$ (more details in Rem. \ref{rem:opt_vs_reg}).

\subsection{Algorithm description: Main Ideas}



{\bf High-level idea behind algorithm design.} The algorithm we propose (\algfewf) is based on using an $(\epsilon,\delta)$-PAC-algorithm known to have (expected) termination time bounded in terms of $\epsilon$ and $\delta$ (a `worst' case termination guarantee not necessarily dependent on instance parameters) as an underlying black-box subroutine. The wrapper algorithm uses the black-box repeatedly, with successively more stringent values of $\epsilon$ and $\delta$, to eliminate suboptimal arms in a phased manner. The termination analysis of the algorithm shows that any suboptimal arm $i \in [n]\sm \{1\}$ survives for about  $O\Big(\frac{1}{\Delta_i^2}\ln \frac{k}{\delta}\Big)$ rounds before being eliminated, which leads to the desired bound of $O\bigg(\sum_{i=2}^{n}\frac{1}{\Delta_i^2}\ln \frac{k}{\delta}\bigg)$ on algorithm's run time performance (with high probability $(1-\delta)$) (Thm. \ref{thm:sc_fewf}).

%\textbf{Main Idea.} The crucial idea behind bringing out this problem dependent complexity term $(\Delta_i)$ lies in using a $(\epsilon,\delta)$-PAC routine with gradually diminishing adaptive $\epsilon$ values, and judge the competency of rest of surviving arms with respect to the $(\epsilon,\delta)$-PAC winner. 
\vspace{-2pt}
{\bf Algorithm description.} The \algm\, algorithm we propose (Alg. \ref{alg:fewf}) runs in phases indexed by $s = 1,2,\ldots$, where each phase $s$ comprises of the following steps.

{\bf Step 1: Finding a good reference item.} It first calls an $(\epsilon_s,\delta_s)$-PAC subroutine (described in Sec. \ref{sec:alg_epsdel} for completeness) with $\epsilon_s = \frac{1}{2^{s+2}}$ and $\delta_s = \frac{\delta}{120s^3}$ to obtain a `reasonably good item' $b_s$---an item that is likely within an $\epsilon_s$ margin of the \bi\, with probability at least $(1-\delta_s)$) and thus a potential \bi. For this we design a new sequential elimination-based algorithm (Alg. \ref{alg:epsdel} in Appendix \ref{app:wiub_div}),  and argue that it finds such a $(\epsilon_s,\delta_s)$-PAC `good item' with {\em instance-dependent} sample complexity (Thm. \ref{lem:up_algep}), which is crucial in the overall analysis. This is an improvement upon the instance-agnostic Algorithm 6 of \cite{SGwin18} whose sample complexity guarantee is not strong enough to be used along with the wrapper. 
%, which otherwise would have blew up the total sample complexity of the main procedure.
%This pivot finding step is crucial proposed

{\bf Step 2: Benchmarking items against the reference item.} After obtaining a candidate good item, the algorithm pairs up the rest of the surviving arms with this good `probe' item $b_s$ and plays each pair multiple times (up to $t_s =  \frac{4}{\epsilon_s^2}\ln \frac{1}{\delta_s} $ rounds), where $\thetsh$ denotes a 'near-accurate' relative score estimate of the \pl\, model for the set $\cB_b$--we use the subroutine \algs\, for estimating $\thetsh$ (see Alg. \ref{alg:algs}, Thm. \ref{thm:algs} in Appendix \ref{app:subrout}). From the winner data obtained in this process, it updates the empirical pairwise win count $w_i$ of each item within any batch $\cB_b$ by applying a rank-breaking idea (see Alg. \ref{alg:updt_win}, Appendix \ref{app:subrout}) .% (the \rb\, subroutine, Algorithm \ref{alg:updt_win}, Appendix \ref{app:alg_fewf}).

{\bf Step 3: Discarding items weaker than the reference item.} Finally, from each group $\cB_b$, the algorithm eliminates all arms whose empirical pairwise win frequency  over the probe item $b_s$ is less than $\frac{1}{2} - \epsilon_s$ (i.e. $\forall i \in \cB_b$ for which $\hat{p}_{i b_s}< \frac{1}{2} - \epsilon_s$, $\hat{p}_{i j}$ being the empirical pairwise preference of item $i$ over $j$ obtained via \rb). The next phase then begins, unless there is only one surviving item left, which is output as the candidate \bi. 

%The details of the $(\epsilon,\delta)$-PAC algorithm is described in Sec. \ref{sec:alg_epsdel}. But before that we briefly describe the concept of \rb\, update below:

\noindent
\textbf{(1). \algep\, subroutine:} Given $\epsilon, \delta \in (0,1)$, this finds an $(\epsilon, \delta)$-\bi\, in $O\Big(\frac{\thetk}{\epsilon^2}\ln \frac{k}{\delta}\Big)$ samples, where $\thetk=\hspace{-8pt} \underset{S \subseteq [n] \mid |S|=k}{\max} \sum_{i \in S}\theta_i$ (See Alg. \ref{alg:epsdel}, Thm. \ref{lem:up_algep} in Appendix \ref{app:wiub_div}). 

\vspace{-5pt}
\begin{center}
\begin{algorithm}[H]
   \caption{\textbf{\algm}}
   \label{alg:algm}
	\begin{algorithmic}[1]
   \STATE {\bfseries input:} Set of items: $[n]$, Confidence term $\delta > 0$, $n_{ij}(1) \leftarrow 0 ~\forall i,j \in [n]$
   \STATE {\bfseries init:}  $\cA_0 \leftarrow [n]$, $t \leftarrow 1$, $s \leftarrow 1$,  
   \WHILE {$|\cA_{s-1}| > 1$}
   \STATE Set $\epsilon_s = \frac{1}{2^{s+2}}$, $\delta_s = \frac{\delta}{120s^3}$
   \STATE $n_i \leftarrow 0$ for all $i \in \cA_{s-1} \sm \{b_s\}$
   \STATE $b_s \leftarrow $ \algep$(\cA_{s-1},k,1,\epsilon_s,\delta_s)$ 
   
   \REPEAT 
   \STATE Play $(\ell_t,r_t) \in \text{argmin}_{i,j \in \cA_{t-1}} \{ n_{ij}(t)\}$
   \STATE For every pair $i,j \in \cA_{t-1}$ define
   \[
   u_{ij}(t) = \hat p_{ij}(t) + \sqrt{\frac{\alpha \log t}{n_{ij}(t)}}
   \]
   \STATE $n_{i_t,j_t}(t+1) \leftarrow n_{i_t,j_t}(t)+1$
   \STATE Choose $k_t \in \text{argmin}_{i \in \cA_{t-1}} \{ n_{ij}(t)\}$
   \STATE Set $\ell_t' \leftarrow b_s$, $r_t' \leftarrow k_t$ and play $(\ell_t',r_t')$
   \STATE if   %Check for RR
   \STATE %Check for Wrapper
   
   \STATE $t \leftarrow t+1$
   
   \UNTIL {(A),(B), or (C) holds good} 
   
   \STATE $\cA_{t+1} = \cA_t \backslash \big\{i \in \cA_t: \exists j \in A_t \ \text{s.t.}\quad  u_{ij}(t) < \frac{1}{2}\big\}$ \,
   
   $\sigma_1\ldots \sigma_{t_s}, ~\forall i,j \in \cB_b$  
   \STATE $\hp_{ij} := \frac{w_{ij}}{w_{ij} + w_{ji}}$ for all $i,j \in \cB_b$
   \STATE \textbf{If} $\exists i \in \cB_b$ s.t. $\hp_{ib_s} < \frac{1}{2} - \epsilon_s$, \textbf{then} $\cA_s \leftarrow \cA_{s} \cup \{i\}$
%   \ENDFOR
	\STATE $s \leftarrow s + 1$
  \ENDWHILE

   \STATE {\bfseries output:} The item remaining in $\cA_s$ 
	\end{algorithmic}
\end{algorithm}
\vspace{-5pt}
\end{center}


\begin{center}
	\begin{algorithm}[H]
		\caption{\textbf{\algep} }
		\label{alg:edpac}
		\begin{algorithmic}[1]
			\STATE {\bfseries Input:} 
			\STATE ~~~ Set of items: $[n]$
			\STATE ~~~ Error bias: $\epsilon >0$, and confidence parameter: $\delta >0$
			\STATE {\bfseries Initialize:} 
			\STATE ~~~ $S \leftarrow [n]$, $\epsilon_0 \leftarrow \frac{\epsilon}{8}$, and $\delta_0 \leftarrow \frac{\delta}{2}$  
			\WHILE{$\ell = 1,2, \ldots$}
			\STATE Set $\delta_\ell \leftarrow \frac{\delta_{\ell-1}}{2}, \epsilon_\ell \leftarrow \frac{3}{4}\epsilon_{\ell-1}$
			\FOR {$g = 1,2, \cdots G$}
			\STATE $\thetg \leftarrow $ \algs$\big(\cG_g,b,\delta_\ell \big)$
			\FOR {$\tau = 1, 2, \ldots t := \left\lceil \frac{32}{\epsilon_l^2} \ln \frac{4}{\delta_\ell} \right\rceil$  }
			\STATE Play the set $\cG_g$ (one round of battle)
			\STATE Receive feedback: The top-$m$ ranking $\bsigma \in \bSigma_{\cG_{g}}^m$ 
			\STATE Update win-count $w_{ij}$ of each item pair $i,j \in \cG_g$
			\ENDFOR 
			%   	\STATE $B_\ell \leftarrow \text{argmax}\{ i \in \cA \mid  \sum_{j \in \cA\setminus\{i'\}}~\1\big(w_{ij} \ge w_{ji}\big) \}$  
			\STATE Estimate pairwise win probabilities: $\forall i,j \in \cG_g \; \hat p_{i,j} = \frac{w_{ij}}{w_{ij}+w_{ji}}$ if $w_{ij}+w_{ji} > 0$, $\hat p_{i,j} = \frac{1}{2}$ otherwise 
			\STATE If $\exists i \in \cG_g$ such that $\hp_{i j} + \frac{\epsilon_\ell}{2} \ge \frac{1}{2}, \, \forall j \in \cG_g$, then set $c_g \leftarrow i$, else select $c_g \leftarrow$ uniformly at random from $\cG_g$. Set $S \leftarrow S \setminus \left( \cG_g \setminus  \{c_g\}\right)$
			\ENDFOR
			\STATE $S \leftarrow S \cup \cR_\ell$
			\IF{$(|S| == 1)$}
			\STATE Break (out of the {\bf while} loop)
			\ELSIF{$|S|\le k$}
			\STATE $S' \leftarrow $ Randomly sample $k-|S|$ items from $[n] \setminus S$, and set $S \leftarrow S \cup S'$, $\epsilon_\ell \leftarrow \frac{2\epsilon}{3}$, $\delta_\ell \leftarrow {\delta}$  
			%	\STATE Initialize pairwise (empirical) win-count $w_{ij} \leftarrow 0$, for each item pair $i,j \in S$
			%	\FOR {$\tau = 1, 2, \ldots t\,(:= \frac{k}{m\epsilon_\ell^2}\ln \frac{2k}{\delta_\ell})$}
			%   	\STATE Play the set $S$ (one round of battle)
			%   	\STATE Receive TR feedback: $\bsigma \in \bSigma_{S^\tau_{m}}$, where $S^\tau_{m} \subseteq S$ such that $|S^\tau_{m}| = m$ 
			%   	\STATE Update win-count $w_{ij}$ of each item pair $i,j \in S$ using \algupdt$(S,\bsigma)$
			%   	\ENDFOR
			%   	\STATE Define $\hat p_{i,j} = \frac{w_i}{w_i+w_j}, \, \forall i,j \in S$
			%   	\STATE \textbf{If} $\exists i \in \cG_g$ such that $\hp_{i j} + \frac{\epsilon}{2} \ge \frac{1}{2}, \, \forall j \in \cG_g$, \textbf{then} set $c_g \leftarrow i$, \textbf{else} select $c_g \leftarrow$ uniformly at random from $\cG_g$, and  Break (go out of the while loop)
			%  \ELSE
			\ENDIF
			\STATE Divide $S$ into $G: = \big \lceil \frac{|S|}{k} \big \rceil$ sets $\cG_1, \cdots \cG_G$ such that $\cup_{j = 1}^{G}\cG_j = S$, $\cG_{j} \cap \cG_{j'} = \emptyset, ~\forall j,j' \in [G], \, |G_j| = k,\, \forall j \in [G-1]$. \textbf{If} $|\cG_{G}| < k$, \textbf{then} set $\cR_{\ell+1} \leftarrow \cG_G$  and $G = G-1$, \textbf{Else} $\cR_1 \leftarrow \emptyset$.
			
			\ENDWHILE
			%   \UNTIL{$(S == \emptyset)$}
			\STATE {\bfseries Output:} $r_*$, the single item remaining in $S$ %: an $\epsilon$-optimal item
		\end{algorithmic}
	\end{algorithm}
	\vspace{-10pt}
\end{center}

\begin{restatable}[\algfewf: Sample Complexity for $(0,\delta)$-PAC Guarantee for \tf]{thm}{scalgfetf}
	\label{thm:sc_fetf}
	With probability at least $(1-\delta)$, \algfewf\, (Algorithm \ref{alg:fewf}) returns the \bi\,  with sample complexity $N_\cA(0,\delta) = O\bigg(\frac{\thetk}{k}\sum_{i = 2}^n\max\Big( 1, \frac{1}{m\Delta_i^2}\Big) \ln\frac{k}{\delta}\Big(\ln \frac{1}{\Delta_i}\Big)\bigg)$. %where $\thetk: = \arg \max_{S \subseteq [n] \mid |S|=k} \sum_{i \in S}\theta_i$.
	%\red{To be corrected.}
\end{restatable}

\begin{rem}
	Following the similar procedure as argued in Sec. \ref{sec:alg_epsdel}, one can easily derive an $(\epsilon,\delta)$-PAC version of \algfetf\, as well, and a similar  guarantee as that of Thm. \ref{thm:sc_fewfep} with a reduction factor $1/m$. We omit the details in the interest of space.
\end{rem}

\newpage %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

\begin{proof}
	As argued, the main idea behind the $\frac{1}{m}$ factor improvement in the sample complexity w.r.t \wf\, (as proved in Thm. \ref{thm:sc_fewf}), lies behind using \rb \, updates (see Alg. \ref{alg:updt_win}) to the general \tf. This actually gives rise to $O(m)$ times additional number of pairwise preferences in comparison to \wf\, which is why in this case it turns out to be sufficient to sample any batch $\cB_b, \forall b \in [B_s]$ for only  $O\big( \frac{1}{m} \big)$ times compared to the earlier case---precisely the reason behind $\frac{1}{m}$-factor improved sample complexity of \algfewf\, for \tf. The rest of the proof argument is mostly similar to that of Thm. \ref{thm:sc_fewf}. We provide the detailed analysis below for the sake of completeness.
	
	%The proof is based on the following four main observations:
	%\begin{enumerate}
	%\item The \bi\, $a^*$ (i.e. item $1$ in our case) is likely to beat the ($\epsilon_s,\delta_s$)-PAC item by sufficiently high margin, for any sub-phase $s= 1,2\ldots$, and hence is never discarded (see Lem. \ref{lem:bistays}).
	%\item With high probability the set of suboptimal items get discarded at a fixed rate once played for sufficiently long duration (see Lem. \ref{lem:nbigoes}).
	%\item The number of occurrences of any sub-optimal item $i$ before it gets discarded is proportional to $O\Big(\frac{1}{\Delta_i^2}\Big)$ which yields the desired sample complexity of the algorithm (see Lem.\ref{lem:sc_item}).
	%\item Lastly we show in Lem. \ref{lem:sc_bbox} that the additional sample complexity incurred due to invoking the subroutine \algep\, at every sub-phase $s$ is orderwise same as the sample complexity incurred by \algfewf\, in the rest of the sub-phase, due to which \algep\, does  contribute to the overall sample complexity of the algorithm modulo some constant factors.
	%\end{enumerate}
	
	We start by proving the correctness of the algorithm, i.e. with high probability $(1-\delta)$, \algfewf\, indeed returns the \bi\,, i.e. item $1$ in our case. Towards this we first prove the following two lemmas: Lem. \ref{lem:bistaystf} and Lem. \ref{lem:nbigoestf}, same as what was derived for Thm. \ref{thm:sc_fewf} as well---However it is important to note that its is due to the \tf\, feedback the exact same guarantees holds in this case as well, even with a $m$-times lesser observed samples.
	
	\begin{restatable}[]{lem}{bistaystf}
		\label{lem:bistaystf}
		With high probability of at least $(1-\frac{\delta}{20})$, item $1$ is never eliminated, i.e. $1 \in \cA_s$ for all sub-phase $s$. More formally, at the end of any sub-phase $s= 1,2,\ldots$, $\hp_{1b_s} > \frac{1}{2} - \epsilon_s$.
	\end{restatable}
	
	\begin{proof}
		Firstly note that at any sub-phase $s$, each batch $b \in B$ within that phase is played for $t_s = \frac{2\thetk}{m\epsilon_s^2}\ln \frac{k}{\delta_s}$ rounds. Now consider the batch $\cB \owns 1$ at any phase $s$. Clearly $b_s \in \cB$ too. Again since $b_s$ is returned by Alg. \ref{alg:epsdel}, by Thm. \ref{lem:up_algep} we know that with probability at least $(1-\delta_s)$, $p_{b_s1} > \frac{1}{2} - \epsilon_s \, \implies \theta_{b_s} > \theta_1 - 4\epsilon$. This further implies $\theta_{b_s} \ge \theta_1 - \frac{1}{2} = \frac{1}{2}$ (since we assume $\theta_1 = 1$, and at any $s,\, \epsilon_s < \frac{1}{8}$). Moreover by Lem. \ref{lem:algs}, we have $\thetsh \ge \frac{\theta_{b_s} +\thets }{\theta_{b_s}} > \frac{\thets + 1}{2}$ (recall we denote $S = \cB_b \sm \{b_s\}$)
		
		Now let us define $w_i$ as number of times item $i \in \cB$ was returned as the winner in $t_s$ rounds and $i_\tau$ be the winner retuned by the environment upon playing $\cB$ for the $\tau^{th}$ round, where $\tau \in [t_s]$.
		Then clearly $Pr(\{1 \in \sigma_\tau\}) = \sum_{j = 1}^{m}Pr\big( \sigma_\tau(j) = 1 \Big) \ge \frac{m\theta_{1}}{\sum_{j \in \cB}\theta_j} = \frac{m}{\theta_{b_s} + \thets} \ge \frac{m}{1+ \thets}, \, \forall \tau \in [t_s]$, as $1 := \arg \max_{i \in \cB}\theta_i$. Hence $\E[w_{1}] = \sum_{\tau = 1}^{t_s}\E[\1(i_\tau = 1)] = \frac{mt_s}{\theta_{b_s} + \thets} \ge \frac{mt_s}{(1+\thets)}$. 
		Now assuming $b_s$ to be indeed an $(\epsilon_s,\delta_s)$-PAC \bi\, and the bound of Lem. \ref{lem:algs} to hold good as well, applying multiplicative Chernoff-Hoeffdings bound on the random variable $w_{1}$, we get that for any $\eta \in (\sqrt{2}\epsilon_s,1]$, 
		
		\begin{align*}
			Pr\Big( w_{1} \le (1-\eta)\E[w_{1}] \Big) & \le \exp\bigg(- \frac{\E[w_{1}]\eta^2}{2}\bigg) \le \exp\bigg(- \frac{mt_s\eta^2}{2(1+\thets)}\bigg) \\
			& = \exp\bigg(- \frac{2\thetsh\eta^2}{2m\epsilon_s^2(1+\thets)}\ln \frac{k}{\delta_s}\bigg)\\
			&\stackrel{(a)}{\le} \exp\bigg(- \frac{2(\thets+1)\eta^2}{4\epsilon_s^2(1+\thets)}\ln \frac{k}{\delta_s}\bigg)\\
			& \le \exp\bigg(- \frac{\eta^2}{2\epsilon_s^2} \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) \le \exp\bigg(- \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) = \frac{\delta_s}{k},
		\end{align*}
		where $(a)$ holds since we proved $\thetsh \ge \frac{\theta_{b_s} +\thets }{\theta_{b_s}} > \frac{\thets + 1}{2}$, and the last inequality holds as $\eta > \epsilon_s\sqrt{2}$.
		
		In particular, note that $\epsilon_s \le \frac{1}{8}$ for any sub-phase $s$, due to which we can safely choose $\eta = \frac{1}{2}$ for any $s$, which gives that with probability at least $\big(1-\frac{\delta_s}{k}\big)$,  $w_{1} > (1-\frac{1}{2})\E[w_{1}] > \frac{mt_s}{2(\theta_{b_s}+\thets)}$, for any subphase $s$.
		
		%====================
		
		Thus above implies that with probability atleast $(1-\frac{\delta_s}{k})$, after $t_s$ rounds we have $w_{1b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)} \implies w_{1b_s} + w_{b_s1} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)}$. Let us denote  $n_{1b_s} = w_{1b_s} + w_{b_s1}$. Then the probability of the event:
		
		\begin{align*}
			Pr\Bigg(  \hp_{1 b_s} & < \frac{1}{2} - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg)
			= Pr\Bigg( \hp_{1 b_s} - \frac{1}{2} < - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)} \Bigg)\\
			& \le Pr\Bigg( \hp_{1 b_s} - p_{1 b_s} < - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)} \Bigg) ~~~(\text{as } \p_{1 b_s} > \frac{1}{2})\\
			& \stackrel{(a)} \le \exp\Big( -2\frac{mt_s}{2(\theta_{b_s}+\thets)}\big({\epsilon_s}\big)^2 \Big) \\
			& \le \exp\Big( -\frac{2m(\theta_{b_s} + \thets)}{m\epsilon_s^2\theta_{b_s}(\theta_{b_s}+\thets)}\big({\epsilon_s}\big)^2 \Big) 
			\le \frac{\delta_s}{k},
		\end{align*}
		
		where the last inequality $(a)$ follows from Lem. \ref{lem:pl_simulator} for $\eta = \epsilon_s$ and $v = \frac{t_s}{2k}$.
		
		Thus under the two assumptions that (1). $b_s$ is indeed an $(\epsilon_s,\delta_s)$-PAC \bi\, and (2). the bound of Lem. \ref{lem:algs} holds good, combining the above two claims, at any sub-phase $s$, we have
		
		\begin{align*}
			& Pr\Bigg(  \hp_{1 b_s} < \frac{1}{2} - \epsilon_s\Bigg)\\
			& = 
			Pr\Bigg(  \hp_{1 b_s} < \frac{1}{2} - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg) + Pr\Bigg(  \hp_{1 b_s} < \frac{1}{2} - \epsilon_s  ,  n_{1 b_s} < \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg)\\
			& \le \frac{\delta_s}{k} + Pr\Bigg( n_{1 b_s} < \frac{mt_s}{2(\theta_{b_s}+\thets)}  \Bigg) \le \frac{2\delta_s}{k} \le \delta_s ~~~(\text{since } k \ge 2)\\
		\end{align*}
		
		Moreover from Thm. \ref{lem:up_algep} and Lem. \ref{lem:algs} we know that the above two assumptions hold with probability at least $(1-2\delta_s)$. Then taking union bound over all sub-phases $s = 1,2, \ldots$, the probability that item $1$ gets eliminated at any round:
		
		\begin{align*}
			Pr\Bigg( \exists s = 1,2, \ldots \text{ s.t. } \hp_{1 b_s} < \frac{1}{2} - \epsilon_s \Bigg) & = \sum_{s = 1}^{\infty}{3\delta_s} = \sum_{s = 1}^{\infty}\frac{3\delta}{120s^3} \le \frac{\delta}{40}\sum_{s = 1}^{\infty}\frac{1}{s^2} \le \frac{\delta}{40}\frac{\pi^2}{6} \le \frac{\delta}{20},
		\end{align*}
		where the first inequality holds since $k \ge 2$.
	\end{proof}
	Recall the notations introduced in the proof of Thm. \ref{thm:sc_fewf}: $\Delta_i = \theta_1-\theta_i$ (Sec. \ref{sec:prb_setup}), $\Delta_{\min} = \min_{i \in [n]\sm\{1\}}\Delta_i$.
	Further $[n]_r := \{ i \in [n] : \frac{1}{2^r} \le \Delta_i < \frac{1}{2^{r-1}} \}$, and $\cA_{r,s}$, i.e. $\cA_{r,s} = [n]_r \cap \cA_s$, for all $s = 1,2, \ldots$.
	Then in this case again we claim:
	
	\begin{restatable}[]{lem}{nbigoestf}
		\label{lem:nbigoestf}
		Assuming that the best arm $1$ is not eliminated at any sub-phase $s = 1,2,\ldots$, then with probability at least $(1-\frac{19\delta}{20})$, for any sub-phase $s \ge r$, $|\cA_{r,s}| \le \frac{2}{19}|\cA_{r,s-1}|$, for any $r = 0,1,2,\ldots \log_2 (\Delta_{\min})$. 
	\end{restatable}
	
	
	\begin{proof}
		Consider any sub-phase $s$, and let us start by noting some properties of $b_s$. Note that by Lem. \ref{lem:up_algep}, with high probability $(1-\delta_s)$, $p_{b_s 1} > \frac{1}{2} - \epsilon_s$. Then this further implies
		
		\begin{align*}
			p_{b_s 1} > \frac{1}{2} - \epsilon_s & \implies \frac{(\theta_{b_s} - \theta_1)}{2(\theta_{b_s} + \theta_1)} > -\epsilon_s\\
			& \implies (\theta_{b_s} - \theta_1) > -2\epsilon_s(\theta_{b_s} + \theta_1) > -4\epsilon_s ~~(\text{as} ~\theta_i \in (0,1)\, \forall i \in [n]\sm\{1\}) 
		\end{align*}  
		
		So we have with probability atleast $(1-\delta_s)$,  $\theta_{b_s} > \theta_1 - 4\epsilon_s = \theta_1 - \frac{1}{2^s}$. 
		
		Now consider any fixed $r = 0,1,2,\ldots \log_2(\Delta_{\min})$. Clearly by definition, for any item $i \in [n]_r$, $\Delta_i = \theta_1 - \theta_i > \frac{1}{2^r}$.
		Then combining the above two claims, we have for any sub-phase $s \ge r$, $\theta_{b_s} > \theta_1 - \frac{1}{2^s} \ge \theta_i + \frac{1}{2^r} - \frac{1}{2^s} > 0 \implies p_{b_si} > \frac{1}{2}$, at any $s \ge r$.
		Moreover note that for any $s \ge 1$, $\epsilon_s > \frac{1}{8}$, so that implies $\theta_{b_s} > \theta_1 - 4\epsilon_s > \frac{1}{2}$.
		
		%====================
		
		Recall that at any sub-phase $s$, each batch within that phase is played for $t_s = \frac{2\thetk}{m\epsilon_s^2}\ln \frac{k}{\delta_s}$ many rounds. Now consider any batch such that $\cB \owns i$ for any $i \in [n]_r$. Of course $b_s \in \cB$ as well, and note that we have shown $p_{b_si} > \frac{1}{2}$ with high probability $(1-\delta_s)$. 
		
		Same as Lem. \ref{lem:bistays}, let us again define $w_i$ as number of times item $i \in \cB$ was returned as the winner in $t_s$ rounds, and $i_\tau$ be the winner retuned by the environment upon playing $\cB$ for the $\tau^{th}$ rounds, where $\tau \in [t_s]$.
		Then given $\theta_{b_s} > \frac{1}{2}$ (as derived earlier), clearly $Pr(\{b_s \in \sigma_\tau\}) = \sum_{j = 1}^{m}Pr\big( \sigma_\tau(j) = b_s \Big) \ge \sum_{j = 0}^{m-1}\frac{\theta_{b_s}}{(\theta_{b_s} + \thets)} = \frac{m\theta_{b_s}}{\theta_{b_s} + \thets}, \, \forall \tau \in [t_s]$. Hence $\E[w_{b_s}] = \sum_{\tau = 1}^{t_s}\E[\1(i_\tau = b_s)] = \frac{m\theta_{b_s}t_s}{(\theta_{b_s} + \thets)}$. 
		Now applying multiplicative Chernoff-Hoeffdings bound on the random variable $w_{b_s}$, we get that for any $\eta \in (\sqrt 2\epsilon_s,1]$, 
		
		\begin{align*}
			Pr\Big( w_{b_s} & \le (1-\eta)\E[w_{b_s}] \mid \theta_{b_s} > \frac{1}{2}, \thetsh > \frac{(\theta_{b_s} + \thets)}{\theta_{b_s}} \Big)\\
			& \le \exp\bigg(- \frac{\E[w_{b_s}]\eta^2}{2}\bigg) \le \exp\bigg(- \frac{m\theta_{b_s}t_s\eta^2}{2(\theta_{b_s} + \thets)}\bigg) \\
			& \le \exp\bigg(- \frac{\eta^2}{2\epsilon_s^2} \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) \le \exp\bigg(- \ln \bigg( \frac{k}{\delta_s} \bigg) \bigg) = \frac{\delta_s}{k},
		\end{align*}
		where the last inequality holds as $\eta > \sqrt 2\epsilon_s$.
		So as a whole, for any $\eta \in (\sqrt 2\epsilon_s,1]$,
		
		\begin{align*}
			& Pr\Big( w_{b_s} \le (1-\eta)\E[w_{b_s}] \Big)\\
			& \le Pr\Big( w_{b_s} \le (1-\eta)\E[w_{b_s}] \mid \theta_{b_s} > \frac{1}{2}, \thetsh > \frac{(\theta_{b_s} + \thets)}{\theta_{b_s}}  \Big)Pr\Big(\theta_{b_s} > \frac{1}{2}\Big) + Pr\Big(\theta_{b_s} < \frac{1}{2},\thetsh > \frac{(\theta_{b_s} + \thets)}{\theta_{b_s}} \Big)\\ 
			& \le \frac{\delta_s}{k} + 2\delta_s
		\end{align*}
		
		In particular, note that $\epsilon_s < \frac{1}{8}$ for any  sub-phase $s$, due to which we can safely choose $\eta = \frac{1}{2}$ for any $s$, which gives that with probability at least $\big(1-\frac{\delta_s}{k}\big)$,  $w_{b_s} > (1-\frac{1}{2})\E[w_{b_s}] > \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}$, for any subphase $s$.
		
		Thus above implies that with probability at least $(1-\frac{\delta_s}{k}-2\delta_s)$, after $t_s$ rounds we have $w_{b_si} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})} \implies w_{ib_s} + w_{b_si} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}$. Let us denote  $n_{ib_s} = w_{ib_s} + w_{b_si}$. Then the probability that item $i$ is not eliminated at any sub-phase $s \ge r$ is:
		
		\begin{align*}
			Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} & - \epsilon_s  ,  n_{i b_s} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}  \Bigg)
			= Pr\Bigg( \hp_{i b_s} - \frac{1}{2} > - \epsilon_s  ,  n_{i b_s} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})} \Bigg)\\
			& \le Pr\Bigg( \hp_{i b_s} - p_{i b_s} > - \epsilon_s  ,  n_{1 b_s} \ge \frac{mt_s \theta_{b_s}}{2 (\thets + \theta_{b_s})}\Bigg) ~~~(\text{as } \p_{i b_s } < \frac{1}{2})\\
			& \stackrel{(a)}\le \exp\Big( -2\frac{mt_s}{2(\thets + \theta_{b_s})}\big({\epsilon_s}\big)^2 \Big)\\
			& \le \exp\Big( -2\frac{m(\thets + \theta_{b_s})}{2m\theta_{b_s}(\thets + \theta_{b_s})}\big({\epsilon_s}\big)^2 \ln \frac{\delta_s}{k}\Big) \le \frac{\delta_s}{k},
		\end{align*}
		
		where $(a)$ follows from Lem. \ref{lem:pl_simulator} for $\eta = \epsilon_s$ and $v = \frac{t_s}{2k}$.
		
		Now combining the above two claims, at any sub-phase $s$, we have:
		
		\begin{align*}
			Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} - \epsilon_s\Bigg) & = 
			Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} - \epsilon_s  ,  n_{i b_s} \ge \frac{t_s}{4k}  \Bigg) + Pr\Bigg(  \hp_{i b_s} > \frac{1}{2} - \epsilon_s  ,  n_{i b_s} < \frac{t_s}{4k}  \Bigg)\\
			& \le \frac{\delta_s}{k} + 2\delta_s + \frac{\delta_s}{k}  \le 3\delta_s ~~~~ (\text{since } k \ge 2)
		\end{align*}
		
		This consequently implies that for any sup-phase $s \ge r$, $\E[|\cA_{r,s}|] \le {3\delta_s}\E[|\cA_{r,s-1}|]$.
		Then applying Markov's Inequality we get:
		
		\begin{align*}
			Pr\Bigg( |\cA_{r,s}| \le \frac{2}{19}|\cA_{r,s-1}| \Bigg)  \le \frac{3\delta_s|\cA_{r,s-1}|}{\frac{2}{19}|\cA_{r,s-1}|} = \frac{57\delta_s}{2}
		\end{align*}
		
		Finally applying union bound over all sub-phases $s= 1,2,\ldots$, and all $r = 1,2, \ldots s$, we get: 
		
		\begin{align*}
			\sum_{s = 1}^{\infty}\sum_{r = 1}^{s}\frac{57\delta_s}{2} = \sum_{s = 1}^{\infty}s\frac{57\delta}{240s^3} = \frac{57\delta}{240}\sum_{s = 1}^{\infty}\frac{1}{s^2} \le \frac{57\delta}{240}\frac{\pi^2}{6} \le \frac{57\delta}{120} \le \frac{19\delta}{20}.
		\end{align*}
		
	\end{proof}
	
	%***************************************************
	
	Thus combining Lem. \ref{lem:bistaystf} and \ref{lem:nbigoestf}, we get that the total failure probability of \algfewf\, is at most $\frac{\delta}{20} + \frac{19\delta}{20} = \delta $.
	
	The remaining thing is to prove the sample complexity bound which crucially follows from a similar claim as proved in Lem. \ref{lem:sc_item}. As before, at any sub-phase $s$, we call the item $b_s$ as the pivot element of phase $s$, then
	
	\begin{restatable}[]{lem}{scitemtf}
		\label{lem:sc_itemtf}
		Assume both Lem. \ref{lem:bistaystf} and Lem. \ref{lem:nbigoestf} holds good and the algorithm does not do a mistake. Consider any item $i \in [n]_r$, for any $r = 1,2, \ldots \log_2(\Delta_{\min})$. Then the total number of times item $i$ gets played as a non-pivot item (i.e. appear in at most one of the $k$-subsets per sub-phase $s$) during the entire run of Alg. \ref{alg:fetf} is $O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}  \Big)$. %\red{Check}
	\end{restatable}
	
	\begin{proof}
		Let us denote the sample complexity of item $i$ (as a non-pivot element) from phase $x$ to $y$ as $\cN^{(i)}_{x,y}$, for any $1 \le x < y < \infty$. Additionally, recalling from Lem. \ref{lem:algs} that $\thetsh \le 7\thetk$, we now prove the claim with the following two case analyses:
		
		\textbf{(Case 1)} Sample complexity till sub-phase $s = r-1$: Note that in the worst case item $i$ can get picked at every sub-phase $s = 1,2,\ldots$ $r-1$, and at every $s$ it is played for $t_s$ rounds. Thus the total number of plays of item $i \in [n]_r$ (as a non-pivot item), till sub-phase $r-1$ becomes:
		
		\[
		\cN^{(i)}_{1,r-1} \le \sum_{s = 1}^{r-1}t_s = \sum_{s = 1}^{r-1}\frac{14\thetk}{m\epsilon_s^2}\ln \frac{k}{\delta_s} = \frac{14\thetk}{m4^{-2}}\sum_{s = 1}^{r-1}(2^s)^2\ln \frac{120ks^3}{\delta} = O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}  \Big)
		\]
		
		\textbf{(Case 2)} Sample complexity from sub-phase $s \ge r$ onwards: Assuming Lem. \ref{lem:nbigoestf} holds good, note that if we define a random variable $I_s$ for any sub-phase $s \ge r$ such that $I_s = \1(i \in \cA_s)$, then clearly $\E[I_{s}] \le \frac{2}{19}\E[I_{s-1}]$ (as follows from the analysis of Lem. \ref{lem:bistaystf}). Then the total expected sample complexity of item $i \in [n]_r$ for round $r, r+1, \ldots \infty$ becomes:
		\begin{align*}
			& \cN^{(i)}_{r,\infty}\le \frac{224\thetk}{m}\sum_{s = r}^{\infty}\bigg(\frac{2}{19}\bigg)^{s-r+1}4^s\ln \frac{k}{\delta_s} = \frac{224\thetk(2^r)^2}{m}\sum_{s = 0}^{\infty}\bigg(\frac{2}{19}\bigg)^{s+1}(2^s)^2\ln \frac{120k(s+r)^3}{\delta}\\
			& = \frac{448}{19m}\thetk(2^r)^2\sum_{s = 0}^{\infty}\bigg(\frac{8}{19}\bigg)^{s}\ln \frac{120k(s+r)^3}{\delta} \\
			& \le \frac{448}{19m}\thetk(2^r)^2\Bigg[\ln \frac{120kr}{\delta}\sum_{s = 0}^{\infty}\bigg(\frac{8}{19}\bigg)^{s} + \sum_{s = 0}^{\infty}\bigg(\frac{8}{19}\bigg)^{s}\ln(120ks)\Bigg] =  O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}  \Big)
		\end{align*}
		
		Combining the two cases above we get $\cN^{(i)}_{1,\infty} = O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}\Big)$ as well, which concludes the proof.
	\end{proof}
	
	Following similar notations as $\cN^{(i)}_{x,y}$, we now denote the number of times any $k$-subset $S \subseteq [n]$ played by the algorithm in sub-phase $x$ to $y$ as $\cN^{(S)}_{x,y}$. Then using Lem. \ref{lem:sc_itemtf}, the total sample complexity of the algorithm \algfewf\, (lets call it algorithm $\cA$) can be written as:
	
	\begin{align}
		\label{eq:sc_fetf}
		\nonumber \cN_\cA(0,\delta) & = \sum_{S \subset [n]\mid |S|=k} \sum_{s=1}^{\infty}\1(S \in \{\cB_1,\ldots, \cB_{B_s}\})t_s = \sum_{i \in [n]} \sum_{s=1}^{\infty}\frac{\1(i \in \cA_s\sm\{b_s\})}{k-1}t_s\\
		\nonumber & = \sum_{s=1}^{\infty} \sum_{i \in [n]}\frac{\1(i \in \cA_s\sm\{b_s\})}{k-1}t_s = \sum_{s=1}^{\infty} \sum_{r=1}^{\log_2(\Delta_{\min})}\sum_{i \in [n]_r}\frac{\1(i \in \cA_s\sm\{b_s\})}{k-1}t_s \\
		\nonumber & = \frac{1}{k-1}\sum_{r=1}^{\log_2(\Delta_{\min})}\sum_{i \in [n]_r}\cN^{(i)}_{1,\infty} ~~(\text{ Lem. \ref{lem:sc_item}})\\
		\nonumber & = \frac{1}{k-1}\sum_{r=1}^{\log_2(\Delta_{\min})}\sum_{i \in [n]_r}O\Big( \frac{(2^r)^2\thetk}{m}\ln \frac{rk}{\delta}\Big) = \frac{\thetk}{k-1}\sum_{r=1}^{\log_2(\Delta_{\min})}|[n]_r|O\Big( \frac{(2^r)^2}{m}\ln \frac{rk}{\delta}\Big) \\
		& = O\Big( \frac{\thetk}{k}\sum_{i=2}^{n}\frac{1}{m\Delta_i^2}\ln \big(\frac{k}{\delta} \ln \frac{1}{\Delta_i} \big) \Big),
	\end{align}
	where the last inequality follows since $2^r < \frac{2}{\Delta_i}$ by definition for all $i \in [n]_r$.
	%Finally the last thing to account for is the additional sample complexity incurred due to calling the subroutine \algep\ at every sub-phase $s$. But following the same argument as of Thm. \ref{thm:sc_fewf}, this is taken care of by Thm. \ref{lem:up_algep}. %, which can easily verified to hold good in this case as well. 
	Finally, same as derived in the proof of Thm. \ref{thm:sc_fewf}, the last thing to account for is the additional sample complexity incurred due to calling the subroutine \algep\ and \algs\, at every sub-phase $s$, which is combinedly known to be of $O\bigg(\frac{|\cA_s|\Theta_[k]}{k} \Big( 1,\frac{1}{(m 2^s)^2}\Big)\ln \frac{k}{\delta} \bigg)$ at any sub-phase $s$ (from Thm. \ref{lem:up_algep} and Cor. \ref{cor:algs}). And using a similar summation as shown above over all $s = 1,2,\ldots \infty$, combined with Lem. \ref{lem:nbigoestf} and using the fact that $2^r < \frac{2}{\Delta_i}$, one can show that the total sample complexity incurred due to the above subroutines is at most $\frac{\Theta_{[k]}}{k}\sum_{i = 2}^{n}\max\big(1,\frac{1}{m \Delta_i^2}\big) \log \frac{k}{\delta})$. Considering the above sample complexity added with the one derived in Eqn. \ref{eq:sc_fetf} finally gives the desired $O\bigg(\frac{\thetk}{k}\sum_{i = 2}^n\max\Big(1,\frac{1}{m \Delta_i^2}\Big) \ln\frac{k}{\delta}\Big(\ln \frac{1}{\Delta_i}\Big)\bigg)$ sample complexity bound of Alg. \ref{alg:fetf}.
\end{proof}

\newpage %%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}
\[	Pr\Big( P(b_s, 1) > 1/2 - \epsilon_s \Big) \geq 1 - \delta_s \]
\end{lem}

\begin{restatable}[]{lem}{bistays}
	\label{lem:bistays}
	With high probability of at least $(1-\frac{\delta}{20})$, item $1$ is never eliminated, i.e. $1 \in \cA_s$ for all sub-phase $s$. More formally, at the end of any sub-phase $s= 1,2,\ldots$, $\hp_{1b_s} > \frac{1}{2} - \epsilon_s$.
\end{restatable}


\textbf{Notations.}
Recall that we defined $\Delta_i = P(1,i) - 1/2$ (Sec. \ref{sec:prb_setup}). We further denote $\Delta_{\min} = \min_{i \in [n]\sm\{1\}}\Delta_i$.
We define the set of arms $[n]_r := \{ i \in [n] : \frac{1}{2^r} \le \Delta_i < \frac{1}{2^{r-1}} \}$, and denote the set of surviving arms in $[n]_r$ at $s^{th}$ sub-phase by $\cA_{r,s}$, i.e. $\cA_{r,s} = [n]_r \cap \cA_s$, for all $s = 1,2, \ldots$.

\begin{restatable}[]{lem}{nbigoes}
	\label{lem:nbigoes}
	Assuming that the best arm $1$ is not eliminated at any sub-phase $s = 1,2,\ldots$, then with probability at least $(1-\frac{19\delta}{20})$, for any sub-phase $s \ge r$, $|\cA_{r,s}| \le \frac{2}{19}|\cA_{r,s-1}|$, for any $r = 0,1,2,\ldots \log_2 (\Delta_{\min})$. 
\end{restatable}


\begin{restatable}[]{lem}{scitem}
	\label{lem:sc_item}
	Assume both Lem. \ref{lem:bistays} and Lem. \ref{lem:nbigoes} holds good and the algorithm does not do a mistake. Consider any item $i \in [n]_r$, for any $r = 1,2, \ldots \log_2(\Delta_{\min})$. Then the total number of times item $i$ gets played as a non-pivot item (i.e. appear in at most one of the $k$-subsets per sub-phase $s$) during the entire run of Alg. \ref{alg:fewf} is $O\Big( (2^r)^2\thetk\ln \frac{rk}{\delta}  \Big)$. %\red{Check}
\end{restatable}


==> apdx-finite-arm.tex <==

\subsection{Proof for~\Cref{thm:fin}}

\begin{restatable}[Regret Analysis of \algfin]{thm}{regalgfin}
  \label{thm:fin}
For any $T >K$, \algfin ($\cA$)\, is $\eps$-DP and its total regret could be bounded as:
  $$\cR_T(\cA) = \tO\left( \sum_{i = 2}^K \frac{\log (KT)}{\Delta(1,i)} + \frac{K}{\epsilon} \right)$$
\end{restatable}

\iffalse%%%%%%%%%%%%
\begin{rem}
Our regret guarantees hold for any preference matrix with SST, STI, which is a slightly general class of preferences compared to assuming $P(i,j) = \sigma(r(i) - r(j))$. 
\end{rem}
\fi%%%%%%%%%%%%%%%%%

\begin{rem}
The regret bound of \algfin\, as described in \cref{thm:fin} is orderwise optimal as this meets both the $\Omega\Big(\sum_{i = 2}^K \frac{\log (KT)}{\Delta(1,i)}\Big)$ non-private
the lower bound of standard $K$-armed dueling bandit as well as the $\Omega(K/\eps)$
privacy lower bound to come in~\Cref{sec:lb}.
\end{rem}

%\iffalse%%%%%%%%%%%%%

\begin{proof}[Prof sketch of \cref{thm:fin}]
The proof is developed based on several lemmas:

\begin{restatable}[]{lem}{unbiasedest}
\label{lem:unbiasedest}
Consider any fixed $n$, subset $\cS \subseteq [K]$ and any $i \in \cS$. Given any item $i \in \cS$, define a random variable $\hcB_n(i):= \frac{1}{n}\sum_{t = 1}^n \1(\text{i wins over a random item in } \cS)$. Then $\E[\hcB_n(i)] = \cB_{S}(i)$.
\end{restatable}


For the privacy proof, we have the following lemma.
\begin{lemma}
\label{lemma:priv-fin}
    Let $\eps \le 1$, $T \ge 1$ and $K\ge1$.
    \Cref{alg:fin} is $\eps$-differentially private.
\end{lemma}
\as{@HA - Reviewers are going to complain why we did not do $(\epsilon,\delta)$-DP, we should do this before arxiv?}

\begin{proof}
    The proof follows from the guarantees of the binary tree mechanism as the output of the algorithm is post-processing of the output of the binary tree mechanism. Note that we have $K$ instantiations of the binary tree mechanism in the algorithm $C^1,\dots,C^k$, thus it is sufficient to show that each $C^1,\dots,C^k$ is $\eps$-DP. 

    We now prove each $C^1,\dots,C^k$ is $\eps$-DP. Note that each user can affect at most two counters. Moreover, the user can contribute only twice to each of these counters: once when adding $+1$ and the other when subtracting $-1$. As $C^i$ is $\eps/4$-DP, we get that each of these counters is $\eps/2$-DP by group privacy, and both counters are $\eps$-DP. The claim follows.
\end{proof}
%
%\noindent
Note \cref{lem:unbiasedest} implies that given any phase $\tau$, $\E[\hcB_{t}(i)] = \cB_{\cS_\tau}(i), ~\forall i \in \cS_\tau$. 

Moreover, due to the binary tree mechanism we have $\hat w_t(i) = w_t(i)  + \zeta_t(i)$,  $\zeta_t(i)$ being a $0$ mean Laplace noise, which gives 
$\E[\hcB_{t}(i)] = \E[\tcB_{t}(i)]$. Combining the results this immediately implies the following corollary:  
\begin{cor}
\label{cor:unbiasedest}
Consider any time step $t$ at a given phase $\tau$. 
Then $\tcB_{t}(i)$ is an unbiased estimate of $\cB_{\cS_{\tau}}(i)$, specifically $E[\tcB_{t}(i)] = \cB_{\cS_\tau}(i), ~\forall i \in \cS_\tau$. %where $\cH_\tau$ denotes the history till the start of phase $\tau$.
\end{cor}
% the noise added by the binary tree mechanism has zero mean. \red{make formal--} since . 

%
\begin{restatable}[]{lem}{estconcs}
\label{lem:est_concs}
For any choice of $\delta \in (0,1/2]$, for all time step $t$ in any phase $\tau$, the true EBS of any arm $i$ is contained within LCB$(\tcB_t(i))$ and UCB$(\tcB_t(i))$, specifically:
\[
\P\big( \exists t \in \text{Phase-}\tau, \exists i \in \cS_\tau, \cB_{\cS_\tau}(i) \notin [\text{LCB}_t(i),\text{UCB}_t(i)] \big) \leq \delta
\]
\end{restatable}
%
\begin{restatable}[]{lem}{winnerstays}
  \label{lem:winnerstays}
 Assuming the concentrations of \cref{lem:est_concs} hold good, i.e. $\forall t \in \text{Phase-}\tau, \text{ and } \forall i \in \cS_\tau, \cB_{\cS_\tau}(i) \in [\text{LCB}_t(i),\text{UCB}_t(i)]$, the best arm $1$ is always a part of surviving set of arms $\cS_{\tau}$ for all phase $\tau \in \{1,2, \ldots K-1\}$.
\end{restatable}
%
\begin{restatable}[]{lem}{loserout}
  \label{lem:loserout}
  Assuming the concentrations of \cref{lem:est_concs} hold good, i.e. $\forall t \in \text{Phase-}\tau, \text{ and } \forall i \in \cS_\tau, \cB_{\cS_\tau}(i) \in [\text{LCB}_t(i),\text{UCB}_t(i)]$, then for any suboptimal arm $i$ can be pulled for at most $\big(\frac{8\log \nicefrac{(KT}{\delta)}}{\Delta(1,i)^2} + \frac{64\log \nicefrac{(KT}{\delta)}\log^{2.5} T}{\Delta(1,i)\epsilon}\big)$ times.
\end{restatable}

\noindent
The proof of the above lemmas are given in \cref{app:fin}. 
Given the results of the above lemmas, \cref{thm:fin} follows immediately setting $\delta = 1/T$:
The first thing to note is that the regret incurred by the learner for playing any item-$i$ ($i \neq 1$) is $r(x_1) - r(x_i) \leq 2\Delta(1,1)$, since by definition $\Delta(1,i):= \sigma(r(x_1) - r(x_i)) - 1/1$. 

Given this observation along with the claim of \cref{lem:loserout}, this implies any suboptimal arm $i \neq 1$ can be pulled  for at most $\big(\frac{8\log \nicefrac{(KT}{\delta)}}{\Delta(1,i)^2} + \frac{64\log \nicefrac{(KT}{\delta)}\log^{2.5} T}{\Delta(1,i)\epsilon}\big)$ times while the learner pays a regret of $2\Delta(1,i)$ for each draw of arm-$i$. Thus the total regret incurred due to the suboptimal arm pulls could be bonded as:
\begin{align*}
\sum_{i = 2}^K&\bigg(\frac{8\log \nicefrac{(KT}{\delta)}}{\Delta(1,i)^2} + \frac{64\log \nicefrac{(KT}{\delta)}\log^{2.5} T}{\Delta(1,i)\epsilon}\bigg) \Delta(1,i) 
 \\
 &\leq \sum_{i = 2}^K \bigg(\frac{16\log (KT)}{\Delta(1,i)} + \frac{128\log(KT)\log^{2.5} T}{\epsilon}\bigg).
\end{align*}
This concludes the regret bound of \cref{thm:fin} with the additional fact of \cref{lem:winnerstays} that with high probability the optimal arm $1$ is never eliminated and hence once the suboptimal arms $i = 2,\ldots K$ are eliminated, the algorithm assigns $\hat i = 1$ and pulls it for the remaining rounds, without incurring any additional regret. Finally $\epsilon$-DP property follows immediately from Lemma~\ref{lemma:priv-fin}.
%\noindent
%\red{NEEDS TO BE REFINED, ensuring $(\epsilon,\delta)$ privacy analysis is not clear ---}Additionally, the privacy guarantees of~\Cref{alg:fin} follow from the guarantees of the binary tree algorithm (Lemma~\ref{lemma:bt}). Any single data point (response $o_t$ at time $t$) is used only in a single binary tree counter $C^{a_t}$, thus the final algorithm is $\eps$-DP as each counter is $\eps$-DP. The complete proof along with the details of the lemmas are given in \cref{app:fin}.
\end{proof}
%\fi %%%%%%%%%%%%%%%%%%%%


==> impact.tex <==
\section*{Impact Statement}
This paper is focused on the development and analysis of theoretical algorithms, with a primary emphasis on design and evaluation. The research undertaken does not entail direct ethical or societal impacts. The primary objective is the advancement of theoretical algorithmic understanding, and as such, the work presented herein is not anticipated to have significant ethical or societal implications.

==> rel_works.tex <==
\subsection{Related Works} 
\label{sec:relworks}

Over the years, Dueling Bandits has been extensively studied with various objectives and generalizations. This includes analyzing the learning rate under different preference structures like total ordering, transitivity, stochastic triangle inequality \cite{falahatgar_nips, BTM}, utility-based preference structures \cite{ailon2014reducing, Busa_pl, SG18, ChenSoda+18}, and general pairwise preference matrices \cite{CDB, SparseDB, Komiyama+16}. Depending on the underlying preference structure, the learner's performance has been assessed against various benchmarks, including best arm identification \cite{SGwin18, Busa_aaai, falahatgar_nips}, top-set detection \cite{Busa_top, SG19}, ranking \cite{Ren+18, SGrank18}, among others.

Some recent works have explored Dueling Bandits in scenarios involving adversarial sequences of preference matrices \cite{gupta2021optimal, Adv_DB, ADB}, robustness to corruptions \cite{agarwal2021stochastic}, extension to potentially infinite arm sets \cite{S21, ContDB}, and contextual scenarios \cite{CDB, SK21}. Another interesting line of work related to Dueling Bandits is its subsetwise generalization, also known as battling bandits \cite{Ren+18, sui2018advancements, Brost+16, ChenSoda+18}.

Despite the widespread surge of interest in learning from preference feedback, surprisingly there has not been a single work on preserving user preferences in the feedback. But this is absolutely important in any real-world systems where human preferences are used for training AI systems. For example, in recommender systems like Netflix and Youtube, the systems are trained based on human preferences, like click data or watch history. However, there is a dire need to keep such sensitive information private, which is however at risk unless the recommender systems ensure a privacy-preserving model during training. Similarly, in various domains of healthcare systems, e.g. 

